Matching with AffNet based rectifications

We consider the problem of two-view matching under significant viewpoint changes with view synthesis. We propose two novel methods, minimizing the view synthesis overhead. The first one, named DenseAffNet, uses dense affine shapes estimates from AffNet, which allows it to partition the image, rectifying each partition with just a single affine map. The second one, named DepthAffNet, combines information from depth maps and affine shapes estimates to produce different sets of rectifying affine maps for different image partitions. DenseAffNet is faster than the state-of-the-art and more accurate on generic scenes. DepthAffNet is on par with the state of the art on scenes containing large planes. The evaluation is performed on 3 public datasets - EVD Dataset, Strong ViewPoint Changes Dataset and IMC Phototourism Dataset.

==> toftrodr_before_squeezing.tex <==
\begin{figure*}[htb]
\centering
\begin{tikzpicture}[
every node/.style={inner sep=2,outer sep=2},
node distance = 2mm and 24mm, auto,
grode/.style={rectangle, draw=black!0, very thin, minimum width=5mm},
]


\node[grode, label={}] (input) {\includegraphics[height=20mm]{imgs/input_image.jpg}};

\node[grode, label={}] (input_sgm) [right=10mm of input] {\includegraphics[height=20mm]{imgs/frame_out.png}};

\node[grode, label={[align=center]below:{\small normals clustering}}] (sphere) [below=of input_sgm] {\includegraphics[height=20mm]{imgs/sphere.png}};

\node[grode, label={}] (red) [right=of input_sgm] {\includegraphics[width=.04\textwidth]{imgs/frame_out_2.png}};
\node[grode] (green) [above=-2mm of red] {\includegraphics[width=.04\textwidth]{imgs/frame_out_3.png}};
\node[grode] (yellow) [below=of red,distance=2mm and 2mm] {\includegraphics[width=.04\textwidth]{imgs/frame_out_1.png}};
\node[grode] (sky) [below=of yellow,distance=2mm and 2mm] {\includegraphics[width=.04\textwidth]{imgs/frame_out_sky.png}};

\node[grode, label={[align=center]left:{\small covering sparse affine shapes} \\ {\small in the space of tilts}}] [above=-1mm and -0mm of green] (covering)
{\includegraphics[height=20mm]{imgs/covering_basic.png}};

\node[grode] (green_right) [right=of green] {\includegraphics[width=.03\textwidth]{imgs/frame_out_3_1.png}};
\node[grode] (green_first) [above=of green_right,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_3_0.png}};
\node[grode] (green_second) [above=of green_first,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_3_2.png}};
\node[grode] (green_third) [below=of green_right,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_3_3.png}};

\node[grode] (red_right) [below=-1mm of green_third,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_2_0.png}};
\node[grode] (red_first) [below=-1mm of red_right,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_2_1.png}};

\node[grode] (yellow_right) [below=-1mm of red_first,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_y_0.png}};
\node[grode] (yellow_first) [below=-1mm of yellow_right,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_y_1.png}};
\node[grode] (yellow_second) [below=-1mm of yellow_first,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_y_2.png}};

\node[grode] (sky_right) [right=of sky,distance=2mm and 2mm] {\includegraphics[width=.03\textwidth]{imgs/frame_out_sky.png}};

\node[grode] (all_back) [right=13cm of input] {\includegraphics[height=20mm]{imgs/frame_out.png}};

\draw[thick, ->] (input) -- (input_sgm) node[midway,above] {};

\draw[thick, ->] (input_sgm) -- (red.west) node[midway,above] {};
\draw[thick, ->] (input_sgm) -- (green.west) node[midway,above] {};
\draw[thick, ->] (input_sgm) -- (yellow.west) node[midway,above] {};
\draw[thick, ->] (input_sgm) -- (sky.west) node[midway,above] {};

\draw[thick, ->] (green) -- (green_right.west) node[midway,above] {{\footnotesize$A_3^1$}};
\draw[thick, ->] (green) -- (green_first.west) node[midway,above] {{\footnotesize$A_2^1$}};
\draw[thick, ->] (green) -- (green_second.west) node[midway,above] {{\footnotesize$A_1^1$}};
\draw[thick, ->] (green) -- (green_third.west) node[midway,above] {{\footnotesize$A_4^1$}};

\draw[thick, ->] (green_right) -- (all_back) node[pos=0.1,above=1mm] {{\footnotesize$(A_3^1)^{-1}$}};
\draw[thick, ->] (green_first) -- (all_back) node[pos=0.1,above=2mm] {{\footnotesize$(A_2^1)^{-1}$}};
\draw[thick, ->] (green_second) -- (all_back) node[pos=0.1,above=3mm] {{\footnotesize$(A_1^1)^{-1}$}};
\draw[thick, ->] (green_third) -- (all_back) node[pos=0.1,above=0mm] {{\footnotesize$(A_4^1)^{-1}$}};

\draw[thick, ->] (red) -- (red_right.west) node[midway,above] {};
\draw[thick, ->] (red) -- (red_first.west) node[midway,above] {};

\draw[thick, ->] (red_right) -- (all_back) node[midway,above] {};
\draw[thick, ->] (red_first) -- (all_back) node[midway,above] {};

\draw[thick, ->] (yellow) -- (yellow_right.west) node[midway,above] {};
\draw[thick, ->] (yellow) -- (yellow_first.west) node[midway,above] {};
\draw[thick, ->] (yellow) -- (yellow_second.west) node[midway,above] {};

\draw[thick, ->] (yellow_right) -- (all_back) node[midway,above] {}; 
\draw[thick, ->] (yellow_first) -- (all_back) node[midway,above] {}; 
\draw[thick, ->] (yellow_second) -- (all_back) node[midway,above] {};

\draw[thick, ->] (sky.east) -- (sky_right.west) node[midway,above] {};
\draw[thick, ->] (sky_right.east) -- (all_back) node[midway,above] {}; 

\end{tikzpicture}
\caption[DepthAffNet rectification]{\textbf{DepthAffNet rectification.} The image is segmented according to clusters of the normals from a depth map. Then each segment is processed independently. Rectification via covering the AffNet shapes is performed on each of them.} 
\label{fig:diagram_depth_affnet}
\end{figure*}

